The evaporation of black holes in supergravity

In supergravity, charged rotating black holes are generically driven towards becoming extremal and supersymmetric through the emission of Hawking radiation. Eventually, as the black hole approaches the BPS bound and is close to becoming supersymmetric, quantum gravity corrections become critical to describing the emission of Hawking radiation, making the QFT in curved spacetime approximation inaccurate. In this paper, we compute how such quantum gravity corrections affect the spectrum of Hawking radiation for black holes in $\mathcal N=2$ supergravity in flatspace. We show that due to such corrections, the spectrum of emitted Hawking radiation for both spin-0 and spin-$1/2$ particles deviates drastically at low temperatures from the naively expected black-body spectrum. Rather remarkably, the spectrum exhibits a discrete emission line from direct transitions from near-BPS to BPS states, providing the first controlled example where the discreteness of the black hole energies is visible in the emitted Hawking radiation. Similar quantum gravity effects drastically modify the absorption cross-section: BPS black holes are transparent to certain frequencies, while near-BPS black holes appear much larger than the semi-classical prediction.

==> mathematica_notebook_N=4/allstates <==
{
 {{(-I)*((h1[l]*(Cos[\[Beta]]*b\[Psi]l1**\[Psi]r1 + 
        E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
        (-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
           b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))/(2*E^l) + 
     I*E^(-1/2*l + (I/2)*\[Alpha] + (I/2)*\[Gamma])*Cos[\[Beta]/2]*
      (-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      (h1[l]/2 + Derivative[1][h1][l]) + b\[Psi]l1**\[Psi]r1*
      ((1/4 - 1/(2*E^l))*h1[l] + Derivative[1][h1][l] + 
       Derivative[2][h1][l])), 1/2, 1/2}, 
  {(-I)*((E^(-l + (I/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]*h1[l]*
       ((-1 + 3*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
        3*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + 3*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))/6 + 
     I*E^(-1/2*l + I*\[Alpha] + I*\[Gamma])*Cos[\[Beta]/2]^2*
      (-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      (h1[l] + Derivative[1][h1][l]) + E^((I/2)*\[Alpha] + (I/2)*\[Gamma])*
      Cos[\[Beta]/2]*b\[Psi]l1**\[Psi]r1*((1 - 1/(3*E^l))*h1[l] + 
       2*Derivative[1][h1][l] + Derivative[2][h1][l])), 1, 1}, 
  {(-I)*((E^(-l + I*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^2*h1[l]*
       ((-1 + 2*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
        4*E^(I*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^2*b\[Psi]l2**\[Psi]r2 + 
        2*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
           b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))/4 + 
     I*E^(-1/2*l + ((3*I)/2)*\[Alpha] + ((3*I)/2)*\[Gamma])*Cos[\[Beta]/2]^3*
      (-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      ((3*h1[l])/2 + Derivative[1][h1][l]) + E^(I*\[Alpha] + I*\[Gamma])*
      Cos[\[Beta]/2]^2*b\[Psi]l1**\[Psi]r1*((9/4 - 1/(4*E^l))*h1[l] + 
       3*Derivative[1][h1][l] + Derivative[2][h1][l])), 3/2, 3/2}, 
  {(-I)*((E^(-l + ((3*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^3*h1[l]*
       ((-3 + 5*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
        5*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + 5*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))/10 + 
     I*E^(-1/2*l + (2*I)*\[Alpha] + (2*I)*\[Gamma])*Cos[\[Beta]/2]^4*
      (-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      (2*h1[l] + Derivative[1][h1][l]) + 
     E^(((3*I)/2)*\[Alpha] + ((3*I)/2)*\[Gamma])*Cos[\[Beta]/2]^3*
      b\[Psi]l1**\[Psi]r1*((4 - 1/(5*E^l))*h1[l] + 4*Derivative[1][h1][l] + 
       Derivative[2][h1][l])), 2, 2}, 
  {(-I)*((E^(-l + (2*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^4*h1[l]*
       ((-2 + 3*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
        3*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + 3*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))/6 + 
     I*E^(-1/2*l + ((5*I)/2)*\[Alpha] + ((5*I)/2)*\[Gamma])*Cos[\[Beta]/2]^5*
      (-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      ((5*h1[l])/2 + Derivative[1][h1][l]) + 
     E^((2*I)*\[Alpha] + (2*I)*\[Gamma])*Cos[\[Beta]/2]^4*b\[Psi]l1**\[Psi]r1*
      ((25/4 - 1/(6*E^l))*h1[l] + 5*Derivative[1][h1][l] + 
       Derivative[2][h1][l])), 5/2, 5/2}, 
  {(-I)*((E^(-l + ((5*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^5*h1[l]*
       ((-5 + 7*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
        7*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + 7*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))/14 + 
     I*E^(-1/2*l + (3*I)*\[Alpha] + (3*I)*\[Gamma])*Cos[\[Beta]/2]^6*
      (-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      (3*h1[l] + Derivative[1][h1][l]) + 
     E^(((5*I)/2)*\[Alpha] + ((5*I)/2)*\[Gamma])*Cos[\[Beta]/2]^5*
      b\[Psi]l1**\[Psi]r1*((9 - 1/(7*E^l))*h1[l] + 6*Derivative[1][h1][l] + 
       Derivative[2][h1][l])), 3, 3}, 
  {(-I)*((E^(-l + (3*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^6*h1[l]*
       ((-3 + 4*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
        4*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + 4*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))/8 + 
     I*E^(-1/2*l + ((7*I)/2)*\[Alpha] + ((7*I)/2)*\[Gamma])*Cos[\[Beta]/2]^7*
      (-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      ((7*h1[l])/2 + Derivative[1][h1][l]) + 
     E^((3*I)*\[Alpha] + (3*I)*\[Gamma])*Cos[\[Beta]/2]^6*b\[Psi]l1**\[Psi]r1*
      ((49/4 - 1/(8*E^l))*h1[l] + 7*Derivative[1][h1][l] + 
       Derivative[2][h1][l])), 7/2, 7/2}, 
  {(-I)*((E^(-l + ((7*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^7*h1[l]*
       ((-7 + 9*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
        9*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + 9*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))/18 + 
     I*E^(-1/2*l + (4*I)*\[Alpha] + (4*I)*\[Gamma])*Cos[\[Beta]/2]^8*
      (-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      (4*h1[l] + Derivative[1][h1][l]) + 
     E^(((7*I)/2)*\[Alpha] + ((7*I)/2)*\[Gamma])*Cos[\[Beta]/2]^7*
      b\[Psi]l1**\[Psi]r1*((16 - 1/(9*E^l))*h1[l] + 8*Derivative[1][h1][l] + 
       Derivative[2][h1][l])), 4, 4}, 
  {(-I)*((E^(-l + (4*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^8*h1[l]*
       ((-4 + 5*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
        5*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + 5*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))/10 + 
     I*E^(-1/2*l + ((9*I)/2)*\[Alpha] + ((9*I)/2)*\[Gamma])*Cos[\[Beta]/2]^9*
      (-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      ((9*h1[l])/2 + Derivative[1][h1][l]) + 
     E^((4*I)*\[Alpha] + (4*I)*\[Gamma])*Cos[\[Beta]/2]^8*b\[Psi]l1**\[Psi]r1*
      ((81/4 - 1/(10*E^l))*h1[l] + 9*Derivative[1][h1][l] + 
       Derivative[2][h1][l])), 9/2, 9/2}, 
  {(-I)*((E^(-l + ((9*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^9*h1[l]*
       ((-9 + 11*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
        11*(E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
           b\[Psi]l2**\[Psi]r2 + (-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
            E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])))/22 + 
     I*E^(-1/2*l + (5*I)*\[Alpha] + (5*I)*\[Gamma])*Cos[\[Beta]/2]^10*
      (-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      (5*h1[l] + Derivative[1][h1][l]) + 
     E^(((9*I)/2)*\[Alpha] + ((9*I)/2)*\[Gamma])*Cos[\[Beta]/2]^9*
      b\[Psi]l1**\[Psi]r1*((25 - 1/(11*E^l))*h1[l] + 
       10*Derivative[1][h1][l] + Derivative[2][h1][l])), 5, 5}, 
  {(-I)*((E^(-l + (5*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^10*h1[l]*
       ((-5 + 6*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
        6*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + 6*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))/12 + 
     I*E^(-1/2*l + ((11*I)/2)*\[Alpha] + ((11*I)/2)*\[Gamma])*
      Cos[\[Beta]/2]^11*(-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      ((11*h1[l])/2 + Derivative[1][h1][l]) + 
     E^((5*I)*\[Alpha] + (5*I)*\[Gamma])*Cos[\[Beta]/2]^10*
      b\[Psi]l1**\[Psi]r1*((121/4 - 1/(12*E^l))*h1[l] + 
       11*Derivative[1][h1][l] + Derivative[2][h1][l])), 11/2, 11/2}, 
  {(-I)*((E^(-l + ((11*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^11*h1[l]*
       ((-11 + 13*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
        13*(E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
           b\[Psi]l2**\[Psi]r2 + (-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
            E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])))/26 + 
     I*E^(-1/2*l + (6*I)*\[Alpha] + (6*I)*\[Gamma])*Cos[\[Beta]/2]^12*
      (-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      (6*h1[l] + Derivative[1][h1][l]) + 
     E^(((11*I)/2)*\[Alpha] + ((11*I)/2)*\[Gamma])*Cos[\[Beta]/2]^11*
      b\[Psi]l1**\[Psi]r1*((36 - 1/(13*E^l))*h1[l] + 
       12*Derivative[1][h1][l] + Derivative[2][h1][l])), 6, 6}, 
  {(-I)*((E^(-l + (6*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^12*h1[l]*
       ((-6 + 7*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
        7*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + 7*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))/14 + 
     I*E^(-1/2*l + ((13*I)/2)*\[Alpha] + ((13*I)/2)*\[Gamma])*
      Cos[\[Beta]/2]^13*(-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      ((13*h1[l])/2 + Derivative[1][h1][l]) + 
     E^((6*I)*\[Alpha] + (6*I)*\[Gamma])*Cos[\[Beta]/2]^12*
      b\[Psi]l1**\[Psi]r1*((169/4 - 1/(14*E^l))*h1[l] + 
       13*Derivative[1][h1][l] + Derivative[2][h1][l])), 13/2, 13/2}, 
  {(-I)*((E^(-l + ((13*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^13*h1[l]*
       ((-13 + 15*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
        15*(E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
           b\[Psi]l2**\[Psi]r2 + (-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
            E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])))/30 + 
     I*E^(-1/2*l + (7*I)*\[Alpha] + (7*I)*\[Gamma])*Cos[\[Beta]/2]^14*
      (-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      (7*h1[l] + Derivative[1][h1][l]) + 
     E^(((13*I)/2)*\[Alpha] + ((13*I)/2)*\[Gamma])*Cos[\[Beta]/2]^13*
      b\[Psi]l1**\[Psi]r1*((49 - 1/(15*E^l))*h1[l] + 
       14*Derivative[1][h1][l] + Derivative[2][h1][l])), 7, 7}, 
  {(-I)*((E^(-l + (7*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^14*h1[l]*
       ((-7 + 8*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
        8*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + 8*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))/16 + 
     I*E^(-1/2*l + ((15*I)/2)*\[Alpha] + ((15*I)/2)*\[Gamma])*
      Cos[\[Beta]/2]^15*(-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      ((15*h1[l])/2 + Derivative[1][h1][l]) + 
     E^((7*I)*\[Alpha] + (7*I)*\[Gamma])*Cos[\[Beta]/2]^14*
      b\[Psi]l1**\[Psi]r1*((225/4 - 1/(16*E^l))*h1[l] + 
       15*Derivative[1][h1][l] + Derivative[2][h1][l])), 15/2, 15/2}, 
  {(-I)*((E^(-l + ((15*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^15*h1[l]*
       ((-15 + 17*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
        17*(E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
           b\[Psi]l2**\[Psi]r2 + (-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
            E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])))/34 + 
     I*E^(-1/2*l + (8*I)*\[Alpha] + (8*I)*\[Gamma])*Cos[\[Beta]/2]^16*
      (-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      (8*h1[l] + Derivative[1][h1][l]) + 
     E^(((15*I)/2)*\[Alpha] + ((15*I)/2)*\[Gamma])*Cos[\[Beta]/2]^15*
      b\[Psi]l1**\[Psi]r1*((64 - 1/(17*E^l))*h1[l] + 
       16*Derivative[1][h1][l] + Derivative[2][h1][l])), 8, 8}, 
  {(-I)*((E^(-l + (8*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^16*h1[l]*
       ((-8 + 9*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
        9*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + 9*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))/18 + 
     I*E^(-1/2*l + ((17*I)/2)*\[Alpha] + ((17*I)/2)*\[Gamma])*
      Cos[\[Beta]/2]^17*(-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      ((17*h1[l])/2 + Derivative[1][h1][l]) + 
     E^((8*I)*\[Alpha] + (8*I)*\[Gamma])*Cos[\[Beta]/2]^16*
      b\[Psi]l1**\[Psi]r1*((289/4 - 1/(18*E^l))*h1[l] + 
       17*Derivative[1][h1][l] + Derivative[2][h1][l])), 17/2, 17/2}, 
  {(-I)*((E^(-l + ((17*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^17*h1[l]*
       ((-17 + 19*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
        19*(E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
           b\[Psi]l2**\[Psi]r2 + (-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
            E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])))/38 + 
     I*E^(-1/2*l + (9*I)*\[Alpha] + (9*I)*\[Gamma])*Cos[\[Beta]/2]^18*
      (-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      (9*h1[l] + Derivative[1][h1][l]) + 
     E^(((17*I)/2)*\[Alpha] + ((17*I)/2)*\[Gamma])*Cos[\[Beta]/2]^17*
      b\[Psi]l1**\[Psi]r1*((81 - 1/(19*E^l))*h1[l] + 
       18*Derivative[1][h1][l] + Derivative[2][h1][l])), 9, 9}, 
  {(-I)*((E^(-l + (9*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^18*h1[l]*
       ((-9 + 10*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
        20*E^(I*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^2*b\[Psi]l2**\[Psi]r2 + 
        10*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
           b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))/20 + 
     I*E^(-1/2*l + ((19*I)/2)*\[Alpha] + ((19*I)/2)*\[Gamma])*
      Cos[\[Beta]/2]^19*(-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      ((19*h1[l])/2 + Derivative[1][h1][l]) + 
     E^((9*I)*\[Alpha] + (9*I)*\[Gamma])*Cos[\[Beta]/2]^18*
      b\[Psi]l1**\[Psi]r1*((361/4 - 1/(20*E^l))*h1[l] + 
       19*Derivative[1][h1][l] + Derivative[2][h1][l])), 19/2, 19/2}, 
  {(-I)*((E^(-l + ((19*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^19*h1[l]*
       ((-19 + 21*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
        21*(E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
           b\[Psi]l2**\[Psi]r2 + (-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
            E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])))/42 + 
     I*E^(-1/2*l + (10*I)*\[Alpha] + (10*I)*\[Gamma])*Cos[\[Beta]/2]^20*
      (-1 + b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)*
      (10*h1[l] + Derivative[1][h1][l]) + 
     E^(((19*I)/2)*\[Alpha] + ((19*I)/2)*\[Gamma])*Cos[\[Beta]/2]^19*
      b\[Psi]l1**\[Psi]r1*((100 - 1/(21*E^l))*h1[l] + 
       20*Derivative[1][h1][l] + Derivative[2][h1][l])), 10, 10}}, 
 {{h1[l]/4 + (h1[l]*b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1)/E^l - 
    I*E^(-1/2*l - (I/2)*(\[Alpha] + \[Gamma]))*
     (Cos[\[Beta]/2]*b\[Psi]l1**\[Psi]r1 + E^(I*(\[Alpha] + \[Gamma]))*
       Cos[\[Beta]/2]*b\[Psi]l2**\[Psi]r2 - 
      (E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2 - E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]/2])*(-1/2*h1[l] + 
      Derivative[1][h1][l]) - Derivative[2][h1][l], 1/2, 0}, 
  {E^(-l + (I/2)*\[Alpha] + (I/2)*\[Gamma])*Cos[\[Beta]/2]*h1[l]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1 - 
    ((I/2)*(Cos[\[Beta]]*b\[Psi]l1**\[Psi]r1 + E^(I*(\[Alpha] + \[Gamma]))*
        (1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
       (-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
          b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*(-h1[l] + Derivative[1][h1][l]))/
     E^(l/2) - ((I/2)*b\[Psi]l1**\[Psi]r1*(h1[l] + Derivative[1][h1][l]))/
     E^(l/2) + E^((I/2)*\[Alpha] + (I/2)*\[Gamma])*Cos[\[Beta]/2]*
     (h1[l] - Derivative[2][h1][l]), 1, 1/2}, 
  {E^(-l + I*\[Alpha] + I*\[Gamma])*Cos[\[Beta]/2]^2*h1[l]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1 - 
    (I/6)*E^(-1/2*l + (I/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]*
     ((-1 + 3*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      3*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      3*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*((-3*h1[l])/2 + 
      Derivative[1][h1][l]) - ((2*I)/3)*E^(-1/2*l + (I/2)*\[Alpha] + 
       (I/2)*\[Gamma])*Cos[\[Beta]/2]*b\[Psi]l1**\[Psi]r1*
     ((3*h1[l])/2 + Derivative[1][h1][l]) + E^(I*\[Alpha] + I*\[Gamma])*
     Cos[\[Beta]/2]^2*((9*h1[l])/4 - Derivative[2][h1][l]), 3/2, 1}, 
  {E^(-l + ((3*I)/2)*\[Alpha] + ((3*I)/2)*\[Gamma])*Cos[\[Beta]/2]^3*h1[l]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1 - 
    (I/4)*E^(-1/2*l + I*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^2*
     ((-1 + 2*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      4*E^(I*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^2*b\[Psi]l2**\[Psi]r2 + 
      2*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*
     (-2*h1[l] + Derivative[1][h1][l]) - 
    ((3*I)/4)*E^(-1/2*l + I*\[Alpha] + I*\[Gamma])*Cos[\[Beta]/2]^2*
     b\[Psi]l1**\[Psi]r1*(2*h1[l] + Derivative[1][h1][l]) + 
    E^(((3*I)/2)*\[Alpha] + ((3*I)/2)*\[Gamma])*Cos[\[Beta]/2]^3*
     (4*h1[l] - Derivative[2][h1][l]), 2, 3/2}, 
  {E^(-l + (2*I)*\[Alpha] + (2*I)*\[Gamma])*Cos[\[Beta]/2]^4*h1[l]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1 - 
    (I/10)*E^(-1/2*l + ((3*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^3*
     ((-3 + 5*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      5*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      5*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*((-5*h1[l])/2 + 
      Derivative[1][h1][l]) - ((4*I)/5)*E^(-1/2*l + ((3*I)/2)*\[Alpha] + 
       ((3*I)/2)*\[Gamma])*Cos[\[Beta]/2]^3*b\[Psi]l1**\[Psi]r1*
     ((5*h1[l])/2 + Derivative[1][h1][l]) + 
    E^((2*I)*\[Alpha] + (2*I)*\[Gamma])*Cos[\[Beta]/2]^4*
     ((25*h1[l])/4 - Derivative[2][h1][l]), 5/2, 2}, 
  {E^(-l + ((5*I)/2)*\[Alpha] + ((5*I)/2)*\[Gamma])*Cos[\[Beta]/2]^5*h1[l]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1 - 
    (I/6)*E^(-1/2*l + (2*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^4*
     ((-2 + 3*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      3*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      3*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*
     (-3*h1[l] + Derivative[1][h1][l]) - 
    ((5*I)/6)*E^(-1/2*l + (2*I)*\[Alpha] + (2*I)*\[Gamma])*Cos[\[Beta]/2]^4*
     b\[Psi]l1**\[Psi]r1*(3*h1[l] + Derivative[1][h1][l]) + 
    E^(((5*I)/2)*\[Alpha] + ((5*I)/2)*\[Gamma])*Cos[\[Beta]/2]^5*
     (9*h1[l] - Derivative[2][h1][l]), 3, 5/2}, 
  {E^(-l + (3*I)*\[Alpha] + (3*I)*\[Gamma])*Cos[\[Beta]/2]^6*h1[l]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1 - 
    (I/14)*E^(-1/2*l + ((5*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^5*
     ((-5 + 7*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      7*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      7*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*((-7*h1[l])/2 + 
      Derivative[1][h1][l]) - ((6*I)/7)*E^(-1/2*l + ((5*I)/2)*\[Alpha] + 
       ((5*I)/2)*\[Gamma])*Cos[\[Beta]/2]^5*b\[Psi]l1**\[Psi]r1*
     ((7*h1[l])/2 + Derivative[1][h1][l]) + 
    E^((3*I)*\[Alpha] + (3*I)*\[Gamma])*Cos[\[Beta]/2]^6*
     ((49*h1[l])/4 - Derivative[2][h1][l]), 7/2, 3}, 
  {E^(-l + ((7*I)/2)*\[Alpha] + ((7*I)/2)*\[Gamma])*Cos[\[Beta]/2]^7*h1[l]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1 - 
    (I/8)*E^(-1/2*l + (3*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^6*
     ((-3 + 4*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      4*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      4*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*
     (-4*h1[l] + Derivative[1][h1][l]) - 
    ((7*I)/8)*E^(-1/2*l + (3*I)*\[Alpha] + (3*I)*\[Gamma])*Cos[\[Beta]/2]^6*
     b\[Psi]l1**\[Psi]r1*(4*h1[l] + Derivative[1][h1][l]) + 
    E^(((7*I)/2)*\[Alpha] + ((7*I)/2)*\[Gamma])*Cos[\[Beta]/2]^7*
     (16*h1[l] - Derivative[2][h1][l]), 4, 7/2}, 
  {E^(-l + (4*I)*\[Alpha] + (4*I)*\[Gamma])*Cos[\[Beta]/2]^8*h1[l]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1 - 
    (I/18)*E^(-1/2*l + ((7*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^7*
     ((-7 + 9*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      9*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      9*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*((-9*h1[l])/2 + 
      Derivative[1][h1][l]) - ((8*I)/9)*E^(-1/2*l + ((7*I)/2)*\[Alpha] + 
       ((7*I)/2)*\[Gamma])*Cos[\[Beta]/2]^7*b\[Psi]l1**\[Psi]r1*
     ((9*h1[l])/2 + Derivative[1][h1][l]) + 
    E^((4*I)*\[Alpha] + (4*I)*\[Gamma])*Cos[\[Beta]/2]^8*
     ((81*h1[l])/4 - Derivative[2][h1][l]), 9/2, 4}, 
  {E^(-l + ((9*I)/2)*\[Alpha] + ((9*I)/2)*\[Gamma])*Cos[\[Beta]/2]^9*h1[l]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1 - 
    (I/10)*E^(-1/2*l + (4*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^8*
     ((-4 + 5*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      5*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      5*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*
     (-5*h1[l] + Derivative[1][h1][l]) - 
    ((9*I)/10)*E^(-1/2*l + (4*I)*\[Alpha] + (4*I)*\[Gamma])*Cos[\[Beta]/2]^8*
     b\[Psi]l1**\[Psi]r1*(5*h1[l] + Derivative[1][h1][l]) + 
    E^(((9*I)/2)*\[Alpha] + ((9*I)/2)*\[Gamma])*Cos[\[Beta]/2]^9*
     (25*h1[l] - Derivative[2][h1][l]), 5, 9/2}, 
  {E^(-l + (5*I)*\[Alpha] + (5*I)*\[Gamma])*Cos[\[Beta]/2]^10*h1[l]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1 - 
    (I/22)*E^(-1/2*l + ((9*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^9*
     ((-9 + 11*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      11*(E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + (-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))*
     ((-11*h1[l])/2 + Derivative[1][h1][l]) - 
    ((10*I)/11)*E^(-1/2*l + ((9*I)/2)*\[Alpha] + ((9*I)/2)*\[Gamma])*
     Cos[\[Beta]/2]^9*b\[Psi]l1**\[Psi]r1*((11*h1[l])/2 + 
      Derivative[1][h1][l]) + E^((5*I)*\[Alpha] + (5*I)*\[Gamma])*
     Cos[\[Beta]/2]^10*((121*h1[l])/4 - Derivative[2][h1][l]), 11/2, 5}, 
  {E^(-l + ((11*I)/2)*\[Alpha] + ((11*I)/2)*\[Gamma])*Cos[\[Beta]/2]^11*h1[l]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1 - 
    (I/12)*E^(-1/2*l + (5*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^10*
     ((-5 + 6*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      6*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      6*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*
     (-6*h1[l] + Derivative[1][h1][l]) - 
    ((11*I)/12)*E^(-1/2*l + (5*I)*\[Alpha] + (5*I)*\[Gamma])*
     Cos[\[Beta]/2]^10*b\[Psi]l1**\[Psi]r1*(6*h1[l] + Derivative[1][h1][l]) + 
    E^(((11*I)/2)*\[Alpha] + ((11*I)/2)*\[Gamma])*Cos[\[Beta]/2]^11*
     (36*h1[l] - Derivative[2][h1][l]), 6, 11/2}, 
  {E^(-l + (6*I)*\[Alpha] + (6*I)*\[Gamma])*Cos[\[Beta]/2]^12*h1[l]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1 - 
    (I/26)*E^(-1/2*l + ((11*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^11*
     ((-11 + 13*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      13*(E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + (-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))*
     ((-13*h1[l])/2 + Derivative[1][h1][l]) - 
    ((12*I)/13)*E^(-1/2*l + ((11*I)/2)*\[Alpha] + ((11*I)/2)*\[Gamma])*
     Cos[\[Beta]/2]^11*b\[Psi]l1**\[Psi]r1*((13*h1[l])/2 + 
      Derivative[1][h1][l]) + E^((6*I)*\[Alpha] + (6*I)*\[Gamma])*
     Cos[\[Beta]/2]^12*((169*h1[l])/4 - Derivative[2][h1][l]), 13/2, 6}, 
  {E^(-l + ((13*I)/2)*\[Alpha] + ((13*I)/2)*\[Gamma])*Cos[\[Beta]/2]^13*h1[l]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1 - 
    (I/14)*E^(-1/2*l + (6*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^12*
     ((-6 + 7*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      7*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      7*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*
     (-7*h1[l] + Derivative[1][h1][l]) - 
    ((13*I)/14)*E^(-1/2*l + (6*I)*\[Alpha] + (6*I)*\[Gamma])*
     Cos[\[Beta]/2]^12*b\[Psi]l1**\[Psi]r1*(7*h1[l] + Derivative[1][h1][l]) + 
    E^(((13*I)/2)*\[Alpha] + ((13*I)/2)*\[Gamma])*Cos[\[Beta]/2]^13*
     (49*h1[l] - Derivative[2][h1][l]), 7, 13/2}, 
  {E^(-l + (7*I)*\[Alpha] + (7*I)*\[Gamma])*Cos[\[Beta]/2]^14*h1[l]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1 - 
    (I/30)*E^(-1/2*l + ((13*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^13*
     ((-13 + 15*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      15*(E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + (-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))*
     ((-15*h1[l])/2 + Derivative[1][h1][l]) - 
    ((14*I)/15)*E^(-1/2*l + ((13*I)/2)*\[Alpha] + ((13*I)/2)*\[Gamma])*
     Cos[\[Beta]/2]^13*b\[Psi]l1**\[Psi]r1*((15*h1[l])/2 + 
      Derivative[1][h1][l]) + E^((7*I)*\[Alpha] + (7*I)*\[Gamma])*
     Cos[\[Beta]/2]^14*((225*h1[l])/4 - Derivative[2][h1][l]), 15/2, 7}, 
  {E^(-l + ((15*I)/2)*\[Alpha] + ((15*I)/2)*\[Gamma])*Cos[\[Beta]/2]^15*h1[l]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1 - 
    (I/16)*E^(-1/2*l + (7*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^14*
     ((-7 + 8*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      8*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      8*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*
     (-8*h1[l] + Derivative[1][h1][l]) - 
    ((15*I)/16)*E^(-1/2*l + (7*I)*\[Alpha] + (7*I)*\[Gamma])*
     Cos[\[Beta]/2]^14*b\[Psi]l1**\[Psi]r1*(8*h1[l] + Derivative[1][h1][l]) + 
    E^(((15*I)/2)*\[Alpha] + ((15*I)/2)*\[Gamma])*Cos[\[Beta]/2]^15*
     (64*h1[l] - Derivative[2][h1][l]), 8, 15/2}, 
  {E^(-l + (8*I)*\[Alpha] + (8*I)*\[Gamma])*Cos[\[Beta]/2]^16*h1[l]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1 - 
    (I/34)*E^(-1/2*l + ((15*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^15*
     ((-15 + 17*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      17*(E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + (-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))*
     ((-17*h1[l])/2 + Derivative[1][h1][l]) - 
    ((16*I)/17)*E^(-1/2*l + ((15*I)/2)*\[Alpha] + ((15*I)/2)*\[Gamma])*
     Cos[\[Beta]/2]^15*b\[Psi]l1**\[Psi]r1*((17*h1[l])/2 + 
      Derivative[1][h1][l]) + E^((8*I)*\[Alpha] + (8*I)*\[Gamma])*
     Cos[\[Beta]/2]^16*((289*h1[l])/4 - Derivative[2][h1][l]), 17/2, 8}, 
  {E^(-l + ((17*I)/2)*\[Alpha] + ((17*I)/2)*\[Gamma])*Cos[\[Beta]/2]^17*h1[l]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1 - 
    (I/18)*E^(-1/2*l + (8*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^16*
     ((-8 + 9*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      9*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      9*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*
     (-9*h1[l] + Derivative[1][h1][l]) - 
    ((17*I)/18)*E^(-1/2*l + (8*I)*\[Alpha] + (8*I)*\[Gamma])*
     Cos[\[Beta]/2]^16*b\[Psi]l1**\[Psi]r1*(9*h1[l] + Derivative[1][h1][l]) + 
    E^(((17*I)/2)*\[Alpha] + ((17*I)/2)*\[Gamma])*Cos[\[Beta]/2]^17*
     (81*h1[l] - Derivative[2][h1][l]), 9, 17/2}, 
  {E^(-l + (9*I)*\[Alpha] + (9*I)*\[Gamma])*Cos[\[Beta]/2]^18*h1[l]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1 - 
    (I/38)*E^(-1/2*l + ((17*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^17*
     ((-17 + 19*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      19*(E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + (-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))*
     ((-19*h1[l])/2 + Derivative[1][h1][l]) - 
    ((18*I)/19)*E^(-1/2*l + ((17*I)/2)*\[Alpha] + ((17*I)/2)*\[Gamma])*
     Cos[\[Beta]/2]^17*b\[Psi]l1**\[Psi]r1*((19*h1[l])/2 + 
      Derivative[1][h1][l]) + E^((9*I)*\[Alpha] + (9*I)*\[Gamma])*
     Cos[\[Beta]/2]^18*((361*h1[l])/4 - Derivative[2][h1][l]), 19/2, 9}, 
  {E^(-l + ((19*I)/2)*\[Alpha] + ((19*I)/2)*\[Gamma])*Cos[\[Beta]/2]^19*h1[l]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1 - 
    (I/20)*E^(-1/2*l + (9*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^18*
     ((-9 + 10*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      20*E^(I*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^2*b\[Psi]l2**\[Psi]r2 + 
      10*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*(-10*h1[l] + 
      Derivative[1][h1][l]) - ((19*I)/20)*
     E^(-1/2*l + (9*I)*\[Alpha] + (9*I)*\[Gamma])*Cos[\[Beta]/2]^18*
     b\[Psi]l1**\[Psi]r1*(10*h1[l] + Derivative[1][h1][l]) + 
    E^(((19*I)/2)*\[Alpha] + ((19*I)/2)*\[Gamma])*Cos[\[Beta]/2]^19*
     (100*h1[l] - Derivative[2][h1][l]), 10, 19/2}}, 
 {{-(h1[l]/E^l) - I*E^(-1/2*l - (I/2)*(\[Alpha] + \[Gamma]))*
     (Cos[\[Beta]/2]*b\[Psi]l1**\[Psi]r1 + E^(I*(\[Alpha] + \[Gamma]))*
       Cos[\[Beta]/2]*b\[Psi]l2**\[Psi]r2 - 
      (E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2 - E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]/2])*(-1/2*h1[l] + 
      Derivative[1][h1][l]) - b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     (h1[l]/4 - Derivative[2][h1][l]), 1/2, 0}, 
  {-(E^(-l + (I/2)*\[Alpha] + (I/2)*\[Gamma])*Cos[\[Beta]/2]*h1[l]) - 
    ((I/2)*(Cos[\[Beta]]*b\[Psi]l1**\[Psi]r1 + E^(I*(\[Alpha] + \[Gamma]))*
        (1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
       (-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
          b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*(-h1[l] + Derivative[1][h1][l]))/
     E^(l/2) - ((I/2)*b\[Psi]l1**\[Psi]r1*(h1[l] + Derivative[1][h1][l]))/
     E^(l/2) - E^((I/2)*\[Alpha] + (I/2)*\[Gamma])*Cos[\[Beta]/2]*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*(h1[l] - Derivative[2][h1][l]), 
   1, 1/2}, {-(E^(-l + I*\[Alpha] + I*\[Gamma])*Cos[\[Beta]/2]^2*h1[l]) - 
    (I/6)*E^(-1/2*l + (I/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]*
     ((-1 + 3*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      3*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      3*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*((-3*h1[l])/2 + 
      Derivative[1][h1][l]) - ((2*I)/3)*E^(-1/2*l + (I/2)*\[Alpha] + 
       (I/2)*\[Gamma])*Cos[\[Beta]/2]*b\[Psi]l1**\[Psi]r1*
     ((3*h1[l])/2 + Derivative[1][h1][l]) - E^(I*\[Alpha] + I*\[Gamma])*
     Cos[\[Beta]/2]^2*b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     ((9*h1[l])/4 - Derivative[2][h1][l]), 3/2, 1}, 
  {-(E^(-l + ((3*I)/2)*\[Alpha] + ((3*I)/2)*\[Gamma])*Cos[\[Beta]/2]^3*
      h1[l]) - (I/4)*E^(-1/2*l + I*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^2*
     ((-1 + 2*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      4*E^(I*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^2*b\[Psi]l2**\[Psi]r2 + 
      2*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*
     (-2*h1[l] + Derivative[1][h1][l]) - 
    ((3*I)/4)*E^(-1/2*l + I*\[Alpha] + I*\[Gamma])*Cos[\[Beta]/2]^2*
     b\[Psi]l1**\[Psi]r1*(2*h1[l] + Derivative[1][h1][l]) - 
    E^(((3*I)/2)*\[Alpha] + ((3*I)/2)*\[Gamma])*Cos[\[Beta]/2]^3*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     (4*h1[l] - Derivative[2][h1][l]), 2, 3/2}, 
  {-(E^(-l + (2*I)*\[Alpha] + (2*I)*\[Gamma])*Cos[\[Beta]/2]^4*h1[l]) - 
    (I/10)*E^(-1/2*l + ((3*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^3*
     ((-3 + 5*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      5*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      5*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*((-5*h1[l])/2 + 
      Derivative[1][h1][l]) - ((4*I)/5)*E^(-1/2*l + ((3*I)/2)*\[Alpha] + 
       ((3*I)/2)*\[Gamma])*Cos[\[Beta]/2]^3*b\[Psi]l1**\[Psi]r1*
     ((5*h1[l])/2 + Derivative[1][h1][l]) - 
    E^((2*I)*\[Alpha] + (2*I)*\[Gamma])*Cos[\[Beta]/2]^4*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*((25*h1[l])/4 - 
      Derivative[2][h1][l]), 5/2, 2}, 
  {-(E^(-l + ((5*I)/2)*\[Alpha] + ((5*I)/2)*\[Gamma])*Cos[\[Beta]/2]^5*
      h1[l]) - (I/6)*E^(-1/2*l + (2*I)*(\[Alpha] + \[Gamma]))*
     Cos[\[Beta]/2]^4*((-2 + 3*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      3*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      3*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*
     (-3*h1[l] + Derivative[1][h1][l]) - 
    ((5*I)/6)*E^(-1/2*l + (2*I)*\[Alpha] + (2*I)*\[Gamma])*Cos[\[Beta]/2]^4*
     b\[Psi]l1**\[Psi]r1*(3*h1[l] + Derivative[1][h1][l]) - 
    E^(((5*I)/2)*\[Alpha] + ((5*I)/2)*\[Gamma])*Cos[\[Beta]/2]^5*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     (9*h1[l] - Derivative[2][h1][l]), 3, 5/2}, 
  {-(E^(-l + (3*I)*\[Alpha] + (3*I)*\[Gamma])*Cos[\[Beta]/2]^6*h1[l]) - 
    (I/14)*E^(-1/2*l + ((5*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^5*
     ((-5 + 7*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      7*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      7*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*((-7*h1[l])/2 + 
      Derivative[1][h1][l]) - ((6*I)/7)*E^(-1/2*l + ((5*I)/2)*\[Alpha] + 
       ((5*I)/2)*\[Gamma])*Cos[\[Beta]/2]^5*b\[Psi]l1**\[Psi]r1*
     ((7*h1[l])/2 + Derivative[1][h1][l]) - 
    E^((3*I)*\[Alpha] + (3*I)*\[Gamma])*Cos[\[Beta]/2]^6*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*((49*h1[l])/4 - 
      Derivative[2][h1][l]), 7/2, 3}, 
  {-(E^(-l + ((7*I)/2)*\[Alpha] + ((7*I)/2)*\[Gamma])*Cos[\[Beta]/2]^7*
      h1[l]) - (I/8)*E^(-1/2*l + (3*I)*(\[Alpha] + \[Gamma]))*
     Cos[\[Beta]/2]^6*((-3 + 4*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      4*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      4*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*
     (-4*h1[l] + Derivative[1][h1][l]) - 
    ((7*I)/8)*E^(-1/2*l + (3*I)*\[Alpha] + (3*I)*\[Gamma])*Cos[\[Beta]/2]^6*
     b\[Psi]l1**\[Psi]r1*(4*h1[l] + Derivative[1][h1][l]) - 
    E^(((7*I)/2)*\[Alpha] + ((7*I)/2)*\[Gamma])*Cos[\[Beta]/2]^7*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     (16*h1[l] - Derivative[2][h1][l]), 4, 7/2}, 
  {-(E^(-l + (4*I)*\[Alpha] + (4*I)*\[Gamma])*Cos[\[Beta]/2]^8*h1[l]) - 
    (I/18)*E^(-1/2*l + ((7*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^7*
     ((-7 + 9*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      9*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      9*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*((-9*h1[l])/2 + 
      Derivative[1][h1][l]) - ((8*I)/9)*E^(-1/2*l + ((7*I)/2)*\[Alpha] + 
       ((7*I)/2)*\[Gamma])*Cos[\[Beta]/2]^7*b\[Psi]l1**\[Psi]r1*
     ((9*h1[l])/2 + Derivative[1][h1][l]) - 
    E^((4*I)*\[Alpha] + (4*I)*\[Gamma])*Cos[\[Beta]/2]^8*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*((81*h1[l])/4 - 
      Derivative[2][h1][l]), 9/2, 4}, 
  {-(E^(-l + ((9*I)/2)*\[Alpha] + ((9*I)/2)*\[Gamma])*Cos[\[Beta]/2]^9*
      h1[l]) - (I/10)*E^(-1/2*l + (4*I)*(\[Alpha] + \[Gamma]))*
     Cos[\[Beta]/2]^8*((-4 + 5*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      5*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      5*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*
     (-5*h1[l] + Derivative[1][h1][l]) - 
    ((9*I)/10)*E^(-1/2*l + (4*I)*\[Alpha] + (4*I)*\[Gamma])*Cos[\[Beta]/2]^8*
     b\[Psi]l1**\[Psi]r1*(5*h1[l] + Derivative[1][h1][l]) - 
    E^(((9*I)/2)*\[Alpha] + ((9*I)/2)*\[Gamma])*Cos[\[Beta]/2]^9*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     (25*h1[l] - Derivative[2][h1][l]), 5, 9/2}, 
  {-(E^(-l + (5*I)*\[Alpha] + (5*I)*\[Gamma])*Cos[\[Beta]/2]^10*h1[l]) - 
    (I/22)*E^(-1/2*l + ((9*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^9*
     ((-9 + 11*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      11*(E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + (-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))*
     ((-11*h1[l])/2 + Derivative[1][h1][l]) - 
    ((10*I)/11)*E^(-1/2*l + ((9*I)/2)*\[Alpha] + ((9*I)/2)*\[Gamma])*
     Cos[\[Beta]/2]^9*b\[Psi]l1**\[Psi]r1*((11*h1[l])/2 + 
      Derivative[1][h1][l]) - E^((5*I)*\[Alpha] + (5*I)*\[Gamma])*
     Cos[\[Beta]/2]^10*b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     ((121*h1[l])/4 - Derivative[2][h1][l]), 11/2, 5}, 
  {-(E^(-l + ((11*I)/2)*\[Alpha] + ((11*I)/2)*\[Gamma])*Cos[\[Beta]/2]^11*
      h1[l]) - (I/12)*E^(-1/2*l + (5*I)*(\[Alpha] + \[Gamma]))*
     Cos[\[Beta]/2]^10*((-5 + 6*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      6*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      6*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*
     (-6*h1[l] + Derivative[1][h1][l]) - 
    ((11*I)/12)*E^(-1/2*l + (5*I)*\[Alpha] + (5*I)*\[Gamma])*
     Cos[\[Beta]/2]^10*b\[Psi]l1**\[Psi]r1*(6*h1[l] + Derivative[1][h1][l]) - 
    E^(((11*I)/2)*\[Alpha] + ((11*I)/2)*\[Gamma])*Cos[\[Beta]/2]^11*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     (36*h1[l] - Derivative[2][h1][l]), 6, 11/2}, 
  {-(E^(-l + (6*I)*\[Alpha] + (6*I)*\[Gamma])*Cos[\[Beta]/2]^12*h1[l]) - 
    (I/26)*E^(-1/2*l + ((11*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^11*
     ((-11 + 13*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      13*(E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + (-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))*
     ((-13*h1[l])/2 + Derivative[1][h1][l]) - 
    ((12*I)/13)*E^(-1/2*l + ((11*I)/2)*\[Alpha] + ((11*I)/2)*\[Gamma])*
     Cos[\[Beta]/2]^11*b\[Psi]l1**\[Psi]r1*((13*h1[l])/2 + 
      Derivative[1][h1][l]) - E^((6*I)*\[Alpha] + (6*I)*\[Gamma])*
     Cos[\[Beta]/2]^12*b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     ((169*h1[l])/4 - Derivative[2][h1][l]), 13/2, 6}, 
  {-(E^(-l + ((13*I)/2)*\[Alpha] + ((13*I)/2)*\[Gamma])*Cos[\[Beta]/2]^13*
      h1[l]) - (I/14)*E^(-1/2*l + (6*I)*(\[Alpha] + \[Gamma]))*
     Cos[\[Beta]/2]^12*((-6 + 7*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      7*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      7*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*
     (-7*h1[l] + Derivative[1][h1][l]) - 
    ((13*I)/14)*E^(-1/2*l + (6*I)*\[Alpha] + (6*I)*\[Gamma])*
     Cos[\[Beta]/2]^12*b\[Psi]l1**\[Psi]r1*(7*h1[l] + Derivative[1][h1][l]) - 
    E^(((13*I)/2)*\[Alpha] + ((13*I)/2)*\[Gamma])*Cos[\[Beta]/2]^13*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     (49*h1[l] - Derivative[2][h1][l]), 7, 13/2}, 
  {-(E^(-l + (7*I)*\[Alpha] + (7*I)*\[Gamma])*Cos[\[Beta]/2]^14*h1[l]) - 
    (I/30)*E^(-1/2*l + ((13*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^13*
     ((-13 + 15*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      15*(E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + (-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))*
     ((-15*h1[l])/2 + Derivative[1][h1][l]) - 
    ((14*I)/15)*E^(-1/2*l + ((13*I)/2)*\[Alpha] + ((13*I)/2)*\[Gamma])*
     Cos[\[Beta]/2]^13*b\[Psi]l1**\[Psi]r1*((15*h1[l])/2 + 
      Derivative[1][h1][l]) - E^((7*I)*\[Alpha] + (7*I)*\[Gamma])*
     Cos[\[Beta]/2]^14*b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     ((225*h1[l])/4 - Derivative[2][h1][l]), 15/2, 7}, 
  {-(E^(-l + ((15*I)/2)*\[Alpha] + ((15*I)/2)*\[Gamma])*Cos[\[Beta]/2]^15*
      h1[l]) - (I/16)*E^(-1/2*l + (7*I)*(\[Alpha] + \[Gamma]))*
     Cos[\[Beta]/2]^14*((-7 + 8*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      8*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      8*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*
     (-8*h1[l] + Derivative[1][h1][l]) - 
    ((15*I)/16)*E^(-1/2*l + (7*I)*\[Alpha] + (7*I)*\[Gamma])*
     Cos[\[Beta]/2]^14*b\[Psi]l1**\[Psi]r1*(8*h1[l] + Derivative[1][h1][l]) - 
    E^(((15*I)/2)*\[Alpha] + ((15*I)/2)*\[Gamma])*Cos[\[Beta]/2]^15*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     (64*h1[l] - Derivative[2][h1][l]), 8, 15/2}, 
  {-(E^(-l + (8*I)*\[Alpha] + (8*I)*\[Gamma])*Cos[\[Beta]/2]^16*h1[l]) - 
    (I/34)*E^(-1/2*l + ((15*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^15*
     ((-15 + 17*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      17*(E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + (-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))*
     ((-17*h1[l])/2 + Derivative[1][h1][l]) - 
    ((16*I)/17)*E^(-1/2*l + ((15*I)/2)*\[Alpha] + ((15*I)/2)*\[Gamma])*
     Cos[\[Beta]/2]^15*b\[Psi]l1**\[Psi]r1*((17*h1[l])/2 + 
      Derivative[1][h1][l]) - E^((8*I)*\[Alpha] + (8*I)*\[Gamma])*
     Cos[\[Beta]/2]^16*b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     ((289*h1[l])/4 - Derivative[2][h1][l]), 17/2, 8}, 
  {-(E^(-l + ((17*I)/2)*\[Alpha] + ((17*I)/2)*\[Gamma])*Cos[\[Beta]/2]^17*
      h1[l]) - (I/18)*E^(-1/2*l + (8*I)*(\[Alpha] + \[Gamma]))*
     Cos[\[Beta]/2]^16*((-8 + 9*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      9*E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*b\[Psi]l2**\[Psi]r2 + 
      9*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*
     (-9*h1[l] + Derivative[1][h1][l]) - 
    ((17*I)/18)*E^(-1/2*l + (8*I)*\[Alpha] + (8*I)*\[Gamma])*
     Cos[\[Beta]/2]^16*b\[Psi]l1**\[Psi]r1*(9*h1[l] + Derivative[1][h1][l]) - 
    E^(((17*I)/2)*\[Alpha] + ((17*I)/2)*\[Gamma])*Cos[\[Beta]/2]^17*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     (81*h1[l] - Derivative[2][h1][l]), 9, 17/2}, 
  {-(E^(-l + (9*I)*\[Alpha] + (9*I)*\[Gamma])*Cos[\[Beta]/2]^18*h1[l]) - 
    (I/38)*E^(-1/2*l + ((17*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^17*
     ((-17 + 19*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      19*(E^(I*(\[Alpha] + \[Gamma]))*(1 + Cos[\[Beta]])*
         b\[Psi]l2**\[Psi]r2 + (-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + 
          E^(I*\[Alpha])*b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]]))*
     ((-19*h1[l])/2 + Derivative[1][h1][l]) - 
    ((18*I)/19)*E^(-1/2*l + ((17*I)/2)*\[Alpha] + ((17*I)/2)*\[Gamma])*
     Cos[\[Beta]/2]^17*b\[Psi]l1**\[Psi]r1*((19*h1[l])/2 + 
      Derivative[1][h1][l]) - E^((9*I)*\[Alpha] + (9*I)*\[Gamma])*
     Cos[\[Beta]/2]^18*b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     ((361*h1[l])/4 - Derivative[2][h1][l]), 19/2, 9}, 
  {-(E^(-l + ((19*I)/2)*\[Alpha] + ((19*I)/2)*\[Gamma])*Cos[\[Beta]/2]^19*
      h1[l]) - (I/20)*E^(-1/2*l + (9*I)*(\[Alpha] + \[Gamma]))*
     Cos[\[Beta]/2]^18*((-9 + 10*Cos[\[Beta]])*b\[Psi]l1**\[Psi]r1 + 
      20*E^(I*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^2*b\[Psi]l2**\[Psi]r2 + 
      10*(-(E^(I*\[Gamma])*b\[Psi]l1**\[Psi]r2) + E^(I*\[Alpha])*
         b\[Psi]l2**\[Psi]r1)*Sin[\[Beta]])*(-10*h1[l] + 
      Derivative[1][h1][l]) - ((19*I)/20)*
     E^(-1/2*l + (9*I)*\[Alpha] + (9*I)*\[Gamma])*Cos[\[Beta]/2]^18*
     b\[Psi]l1**\[Psi]r1*(10*h1[l] + Derivative[1][h1][l]) - 
    E^(((19*I)/2)*\[Alpha] + ((19*I)/2)*\[Gamma])*Cos[\[Beta]/2]^19*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     (100*h1[l] - Derivative[2][h1][l]), 10, 19/2}}, 
 {0, {(h1[l] - Derivative[1][h1][l])/E^(l/2) + 
    (b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
      (-h1[l] + Derivative[1][h1][l]))/E^(l/2) + 
    (I/2)*E^(-l - (I/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]*
     b\[Psi]l1**\[Psi]r1*((-2 + E^l*(-1 + ss^2))*h1[l] + 
      2*E^l*Derivative[1][h1][l]) + 
    (I/2)*E^(-l + (I/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]*
     b\[Psi]l2**\[Psi]r2*((-2 + E^l*(-1 + ss^2))*h1[l] + 
      2*E^l*Derivative[1][h1][l]) - 
    (I/2)*E^(-l - (I/2)*(\[Alpha] - \[Gamma]))*b\[Psi]l1**\[Psi]r2*
     Sin[\[Beta]/2]*((-2 + E^l*(-1 + ss^2))*h1[l] + 
      2*E^l*Derivative[1][h1][l]) + 
    (I/2)*E^(-l + (I/2)*(\[Alpha] - \[Gamma]))*b\[Psi]l2**\[Psi]r1*
     Sin[\[Beta]/2]*((-2 + E^l*(-1 + ss^2))*h1[l] + 
      2*E^l*Derivative[1][h1][l]), 1, 0}, 
  {(E^(-1/2*l + (I/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]*
      (3*h1[l] - 2*Derivative[1][h1][l]))/2 - 
    (E^(-1/2*l + (I/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]*
      b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
      (3*h1[l] - 2*Derivative[1][h1][l]))/2 + 
    (I/6)*E^(-l + I*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^2*
     b\[Psi]l2**\[Psi]r2*((-6 + E^l*(-9 + 4*ss^2))*h1[l] + 
      12*E^l*Derivative[1][h1][l]) - (I/12)*E^(-l + I*\[Gamma])*
     b\[Psi]l1**\[Psi]r2*Sin[\[Beta]]*((-6 + E^l*(-9 + 4*ss^2))*h1[l] + 
      12*E^l*Derivative[1][h1][l]) + (I/12)*E^(-l + I*\[Alpha])*
     b\[Psi]l2**\[Psi]r1*Sin[\[Beta]]*((-6 + E^l*(-9 + 4*ss^2))*h1[l] + 
      12*E^l*Derivative[1][h1][l]) + b\[Psi]l1**\[Psi]r1*
     (((I/12)*(-6 + (-6 + E^l*(-9 + 4*ss^2))*Cos[\[Beta]])*h1[l])/E^l + 
      I*Cos[\[Beta]]*Derivative[1][h1][l]), 3/2, 1/2}, 
  {E^(-1/2*l + I*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^2*
     (2*h1[l] - Derivative[1][h1][l]) - E^(-1/2*l + I*(\[Alpha] + \[Gamma]))*
     Cos[\[Beta]/2]^2*b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     (2*h1[l] - Derivative[1][h1][l]) + 
    (I/4)*E^(-l + ((3*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^3*
     b\[Psi]l2**\[Psi]r2*((-4 + 3*E^l*(-4 + ss^2))*h1[l] + 
      12*E^l*Derivative[1][h1][l]) - 
    (I/16)*E^(-l + (I/2)*(\[Alpha] + 3*\[Gamma]))*Csc[\[Beta]/2]*
     b\[Psi]l1**\[Psi]r2*Sin[\[Beta]]^2*((-4 + 3*E^l*(-4 + ss^2))*h1[l] + 
      12*E^l*Derivative[1][h1][l]) + 
    (I/16)*E^(-l + (I/2)*(3*\[Alpha] + \[Gamma]))*Csc[\[Beta]/2]*
     b\[Psi]l2**\[Psi]r1*Sin[\[Beta]]^2*((-4 + 3*E^l*(-4 + ss^2))*h1[l] + 
      12*E^l*Derivative[1][h1][l]) + 
    (I/8)*E^(-l + (I/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]*
     b\[Psi]l1**\[Psi]r1*((-4 - E^l*(-4 + ss^2) + (-4 + 3*E^l*(-4 + ss^2))*
         Cos[\[Beta]])*h1[l] + 4*E^l*(-1 + 3*Cos[\[Beta]])*
       Derivative[1][h1][l]), 2, 1}, 
  {(E^(-1/2*l + ((3*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^3*
      (5*h1[l] - 2*Derivative[1][h1][l]))/2 - 
    (E^(-1/2*l + ((3*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^3*
      b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
      (5*h1[l] - 2*Derivative[1][h1][l]))/2 + 
    (I/5)*E^(-l + (2*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^4*
     b\[Psi]l2**\[Psi]r2*((-5 + E^l*(-25 + 4*ss^2))*h1[l] + 
      20*E^l*Derivative[1][h1][l]) - 
    (I/40)*E^(-l + I*(\[Alpha] + 2*\[Gamma]))*Csc[\[Beta]/2]^2*
     b\[Psi]l1**\[Psi]r2*Sin[\[Beta]]^3*((-5 + E^l*(-25 + 4*ss^2))*h1[l] + 
      20*E^l*Derivative[1][h1][l]) + 
    (I/40)*E^(-l + I*(2*\[Alpha] + \[Gamma]))*Csc[\[Beta]/2]^2*
     b\[Psi]l2**\[Psi]r1*Sin[\[Beta]]^3*((-5 + E^l*(-25 + 4*ss^2))*h1[l] + 
      20*E^l*Derivative[1][h1][l]) + (I/20)*E^(-l + I*(\[Alpha] + \[Gamma]))*
     Cos[\[Beta]/2]^2*b\[Psi]l1**\[Psi]r1*
     ((-10 + E^l*(25 - 4*ss^2) + 2*(-5 + E^l*(-25 + 4*ss^2))*Cos[\[Beta]])*
       h1[l] + 20*E^l*(-1 + 2*Cos[\[Beta]])*Derivative[1][h1][l]), 5/2, 3/2}, 
  {E^(-1/2*l + (2*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^4*
     (3*h1[l] - Derivative[1][h1][l]) - 
    E^(-1/2*l + (2*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^4*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     (3*h1[l] - Derivative[1][h1][l]) + 
    (I/6)*E^(-l + ((5*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^5*
     b\[Psi]l2**\[Psi]r2*((-6 + 5*E^l*(-9 + ss^2))*h1[l] + 
      30*E^l*Derivative[1][h1][l]) - 
    (I/96)*E^(-l + (I/2)*(3*\[Alpha] + 5*\[Gamma]))*Csc[\[Beta]/2]^3*
     b\[Psi]l1**\[Psi]r2*Sin[\[Beta]]^4*((-6 + 5*E^l*(-9 + ss^2))*h1[l] + 
      30*E^l*Derivative[1][h1][l]) + 
    (I/96)*E^(-l + (I/2)*(5*\[Alpha] + 3*\[Gamma]))*Csc[\[Beta]/2]^3*
     b\[Psi]l2**\[Psi]r1*Sin[\[Beta]]^4*((-6 + 5*E^l*(-9 + ss^2))*h1[l] + 
      30*E^l*Derivative[1][h1][l]) + 
    (I/12)*E^(-l + ((3*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^3*
     b\[Psi]l1**\[Psi]r1*((-3*(2 + E^l*(-9 + ss^2)) + 
        (-6 + 5*E^l*(-9 + ss^2))*Cos[\[Beta]])*h1[l] + 
      6*E^l*(-3 + 5*Cos[\[Beta]])*Derivative[1][h1][l]), 3, 2}, 
  {(E^(-1/2*l + ((5*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^5*
      (7*h1[l] - 2*Derivative[1][h1][l]))/2 - 
    (E^(-1/2*l + ((5*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^5*
      b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
      (7*h1[l] - 2*Derivative[1][h1][l]))/2 + 
    (I/14)*E^(-l + (3*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^6*
     b\[Psi]l2**\[Psi]r2*((-14 + 3*E^l*(-49 + 4*ss^2))*h1[l] + 
      84*E^l*Derivative[1][h1][l]) - 
    (I/448)*E^(-l + (2*I)*\[Alpha] + (3*I)*\[Gamma])*Csc[\[Beta]/2]^4*
     b\[Psi]l1**\[Psi]r2*Sin[\[Beta]]^5*((-14 + 3*E^l*(-49 + 4*ss^2))*h1[l] + 
      84*E^l*Derivative[1][h1][l]) + 
    (I/448)*E^(-l + (3*I)*\[Alpha] + (2*I)*\[Gamma])*Csc[\[Beta]/2]^4*
     b\[Psi]l2**\[Psi]r1*Sin[\[Beta]]^5*((-14 + 3*E^l*(-49 + 4*ss^2))*h1[l] + 
      84*E^l*Derivative[1][h1][l]) + 
    (I/28)*E^(-l + (2*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^4*
     b\[Psi]l1**\[Psi]r1*((-14 + E^l*(98 - 8*ss^2) + 
        (-14 + 3*E^l*(-49 + 4*ss^2))*Cos[\[Beta]])*h1[l] + 
      28*E^l*(-2 + 3*Cos[\[Beta]])*Derivative[1][h1][l]), 7/2, 5/2}, 
  {E^(-1/2*l + (3*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^6*
     (4*h1[l] - Derivative[1][h1][l]) - 
    E^(-1/2*l + (3*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^6*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     (4*h1[l] - Derivative[1][h1][l]) + 
    (I/8)*E^(-l + ((7*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^7*
     b\[Psi]l2**\[Psi]r2*((-8 + 7*E^l*(-16 + ss^2))*h1[l] + 
      56*E^l*Derivative[1][h1][l]) - 
    (I/512)*E^(-l + (I/2)*(5*\[Alpha] + 7*\[Gamma]))*Csc[\[Beta]/2]^5*
     b\[Psi]l1**\[Psi]r2*Sin[\[Beta]]^6*((-8 + 7*E^l*(-16 + ss^2))*h1[l] + 
      56*E^l*Derivative[1][h1][l]) + 
    (I/512)*E^(-l + (I/2)*(7*\[Alpha] + 5*\[Gamma]))*Csc[\[Beta]/2]^5*
     b\[Psi]l2**\[Psi]r1*Sin[\[Beta]]^6*((-8 + 7*E^l*(-16 + ss^2))*h1[l] + 
      56*E^l*Derivative[1][h1][l]) + 
    (I/16)*E^(-l + ((5*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^5*
     b\[Psi]l1**\[Psi]r1*((-8 - 5*E^l*(-16 + ss^2) + 
        (-8 + 7*E^l*(-16 + ss^2))*Cos[\[Beta]])*h1[l] + 
      8*E^l*(-5 + 7*Cos[\[Beta]])*Derivative[1][h1][l]), 4, 3}, 
  {(E^(-1/2*l + ((7*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^7*
      (9*h1[l] - 2*Derivative[1][h1][l]))/2 - 
    (E^(-1/2*l + ((7*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^7*
      b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
      (9*h1[l] - 2*Derivative[1][h1][l]))/2 + 
    (I/9)*E^(-l + (4*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^8*
     b\[Psi]l2**\[Psi]r2*((-9 + 2*E^l*(-81 + 4*ss^2))*h1[l] + 
      72*E^l*Derivative[1][h1][l]) - 
    (I/1152)*E^(-l + (3*I)*\[Alpha] + (4*I)*\[Gamma])*Csc[\[Beta]/2]^6*
     b\[Psi]l1**\[Psi]r2*Sin[\[Beta]]^7*((-9 + 2*E^l*(-81 + 4*ss^2))*h1[l] + 
      72*E^l*Derivative[1][h1][l]) + 
    (I/1152)*E^(-l + (4*I)*\[Alpha] + (3*I)*\[Gamma])*Csc[\[Beta]/2]^6*
     b\[Psi]l2**\[Psi]r1*Sin[\[Beta]]^7*((-9 + 2*E^l*(-81 + 4*ss^2))*h1[l] + 
      72*E^l*Derivative[1][h1][l]) + 
    (I/36)*E^(-l + (3*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^6*
     b\[Psi]l1**\[Psi]r1*((-3*(6 + E^l*(-81 + 4*ss^2)) + 
        2*(-9 + 2*E^l*(-81 + 4*ss^2))*Cos[\[Beta]])*h1[l] + 
      36*E^l*(-3 + 4*Cos[\[Beta]])*Derivative[1][h1][l]), 9/2, 7/2}, 
  {E^(-1/2*l + (4*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^8*
     (5*h1[l] - Derivative[1][h1][l]) - 
    E^(-1/2*l + (4*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^8*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     (5*h1[l] - Derivative[1][h1][l]) + 
    (I/10)*E^(-l + ((9*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^9*
     b\[Psi]l2**\[Psi]r2*((-10 + 9*E^l*(-25 + ss^2))*h1[l] + 
      90*E^l*Derivative[1][h1][l]) - 
    (I/10)*E^(-l + (I/2)*(7*\[Alpha] + 9*\[Gamma]))*Cos[\[Beta]/2]^8*
     b\[Psi]l1**\[Psi]r2*Sin[\[Beta]/2]*((-10 + 9*E^l*(-25 + ss^2))*h1[l] + 
      90*E^l*Derivative[1][h1][l]) + 
    (I/2560)*E^(-l + (I/2)*(9*\[Alpha] + 7*\[Gamma]))*Csc[\[Beta]/2]^7*
     b\[Psi]l2**\[Psi]r1*Sin[\[Beta]]^8*((-10 + 9*E^l*(-25 + ss^2))*h1[l] + 
      90*E^l*Derivative[1][h1][l]) + 
    (I/20)*E^(-l + ((7*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^7*
     b\[Psi]l1**\[Psi]r1*((-10 - 7*E^l*(-25 + ss^2) + 
        (-10 + 9*E^l*(-25 + ss^2))*Cos[\[Beta]])*h1[l] + 
      10*E^l*(-7 + 9*Cos[\[Beta]])*Derivative[1][h1][l]), 5, 4}, 
  {(E^(-1/2*l + ((9*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^9*
      (11*h1[l] - 2*Derivative[1][h1][l]))/2 - 
    (E^(-1/2*l + ((9*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^9*
      b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
      (11*h1[l] - 2*Derivative[1][h1][l]))/2 + 
    (I/22)*E^(-l + (5*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^10*
     b\[Psi]l2**\[Psi]r2*((-22 + 5*E^l*(-121 + 4*ss^2))*h1[l] + 
      220*E^l*Derivative[1][h1][l]) - 
    (I/22)*E^(-l + (4*I)*\[Alpha] + (5*I)*\[Gamma])*Cos[\[Beta]/2]^9*
     b\[Psi]l1**\[Psi]r2*Sin[\[Beta]/2]*((-22 + 5*E^l*(-121 + 4*ss^2))*
       h1[l] + 220*E^l*Derivative[1][h1][l]) + 
    (I/22)*E^(-l + (5*I)*\[Alpha] + (4*I)*\[Gamma])*Cos[\[Beta]/2]^9*
     b\[Psi]l2**\[Psi]r1*Sin[\[Beta]/2]*((-22 + 5*E^l*(-121 + 4*ss^2))*
       h1[l] + 220*E^l*Derivative[1][h1][l]) + 
    (I/44)*E^(-l + (4*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^8*
     b\[Psi]l1**\[Psi]r1*((-22 + E^l*(484 - 16*ss^2) + 
        (-22 + 5*E^l*(-121 + 4*ss^2))*Cos[\[Beta]])*h1[l] + 
      44*E^l*(-4 + 5*Cos[\[Beta]])*Derivative[1][h1][l]), 11/2, 9/2}, 
  {E^(-1/2*l + (5*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^10*
     (6*h1[l] - Derivative[1][h1][l]) - 
    E^(-1/2*l + (5*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^10*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     (6*h1[l] - Derivative[1][h1][l]) + 
    (I/12)*E^(-l + ((11*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^11*
     b\[Psi]l2**\[Psi]r2*((-12 + 11*E^l*(-36 + ss^2))*h1[l] + 
      132*E^l*Derivative[1][h1][l]) - 
    (I/12)*E^(-l + (I/2)*(9*\[Alpha] + 11*\[Gamma]))*Cos[\[Beta]/2]^10*
     b\[Psi]l1**\[Psi]r2*Sin[\[Beta]/2]*((-12 + 11*E^l*(-36 + ss^2))*h1[l] + 
      132*E^l*Derivative[1][h1][l]) + 
    (I/12)*E^(-l + (I/2)*(11*\[Alpha] + 9*\[Gamma]))*Cos[\[Beta]/2]^10*
     b\[Psi]l2**\[Psi]r1*Sin[\[Beta]/2]*((-12 + 11*E^l*(-36 + ss^2))*h1[l] + 
      132*E^l*Derivative[1][h1][l]) + 
    (I/24)*E^(-l + ((9*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^9*
     b\[Psi]l1**\[Psi]r1*((-12 - 9*E^l*(-36 + ss^2) + 
        (-12 + 11*E^l*(-36 + ss^2))*Cos[\[Beta]])*h1[l] + 
      12*E^l*(-9 + 11*Cos[\[Beta]])*Derivative[1][h1][l]), 6, 5}, 
  {(E^(-1/2*l + ((11*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^11*
      (13*h1[l] - 2*Derivative[1][h1][l]))/2 - 
    (E^(-1/2*l + ((11*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^11*
      b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
      (13*h1[l] - 2*Derivative[1][h1][l]))/2 + 
    (I/13)*E^(-l + (6*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^12*
     b\[Psi]l2**\[Psi]r2*((-13 + 3*E^l*(-169 + 4*ss^2))*h1[l] + 
      156*E^l*Derivative[1][h1][l]) - 
    (I/13)*E^(-l + (5*I)*\[Alpha] + (6*I)*\[Gamma])*Cos[\[Beta]/2]^11*
     b\[Psi]l1**\[Psi]r2*Sin[\[Beta]/2]*((-13 + 3*E^l*(-169 + 4*ss^2))*
       h1[l] + 156*E^l*Derivative[1][h1][l]) + 
    (I/13)*E^(-l + (6*I)*\[Alpha] + (5*I)*\[Gamma])*Cos[\[Beta]/2]^11*
     b\[Psi]l2**\[Psi]r1*Sin[\[Beta]/2]*((-13 + 3*E^l*(-169 + 4*ss^2))*
       h1[l] + 156*E^l*Derivative[1][h1][l]) + 
    (I/52)*E^(-l + (5*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^10*
     b\[Psi]l1**\[Psi]r1*((-26 + E^l*(845 - 20*ss^2) + 
        2*(-13 + 3*E^l*(-169 + 4*ss^2))*Cos[\[Beta]])*h1[l] + 
      52*E^l*(-5 + 6*Cos[\[Beta]])*Derivative[1][h1][l]), 13/2, 11/2}, 
  {E^(-1/2*l + (6*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^12*
     (7*h1[l] - Derivative[1][h1][l]) - 
    E^(-1/2*l + (6*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^12*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     (7*h1[l] - Derivative[1][h1][l]) + 
    (I/14)*E^(-l + ((13*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^13*
     b\[Psi]l2**\[Psi]r2*((-14 + 13*E^l*(-49 + ss^2))*h1[l] + 
      182*E^l*Derivative[1][h1][l]) - 
    (I/14)*E^(-l + (I/2)*(11*\[Alpha] + 13*\[Gamma]))*Cos[\[Beta]/2]^12*
     b\[Psi]l1**\[Psi]r2*Sin[\[Beta]/2]*((-14 + 13*E^l*(-49 + ss^2))*h1[l] + 
      182*E^l*Derivative[1][h1][l]) + 
    (I/14)*E^(-l + (I/2)*(13*\[Alpha] + 11*\[Gamma]))*Cos[\[Beta]/2]^12*
     b\[Psi]l2**\[Psi]r1*Sin[\[Beta]/2]*((-14 + 13*E^l*(-49 + ss^2))*h1[l] + 
      182*E^l*Derivative[1][h1][l]) + 
    (I/28)*E^(-l + ((11*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^11*
     b\[Psi]l1**\[Psi]r1*((-14 - 11*E^l*(-49 + ss^2) + 
        (-14 + 13*E^l*(-49 + ss^2))*Cos[\[Beta]])*h1[l] + 
      14*E^l*(-11 + 13*Cos[\[Beta]])*Derivative[1][h1][l]), 7, 6}, 
  {(E^(-1/2*l + ((13*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^13*
      (15*h1[l] - 2*Derivative[1][h1][l]))/2 - 
    (E^(-1/2*l + ((13*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^13*
      b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
      (15*h1[l] - 2*Derivative[1][h1][l]))/2 + 
    (I/30)*E^(-l + (7*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^14*
     b\[Psi]l2**\[Psi]r2*((-30 + 7*E^l*(-225 + 4*ss^2))*h1[l] + 
      420*E^l*Derivative[1][h1][l]) - 
    (I/30)*E^(-l + (6*I)*\[Alpha] + (7*I)*\[Gamma])*Cos[\[Beta]/2]^13*
     b\[Psi]l1**\[Psi]r2*Sin[\[Beta]/2]*((-30 + 7*E^l*(-225 + 4*ss^2))*
       h1[l] + 420*E^l*Derivative[1][h1][l]) + 
    (I/30)*E^(-l + (7*I)*\[Alpha] + (6*I)*\[Gamma])*Cos[\[Beta]/2]^13*
     b\[Psi]l2**\[Psi]r1*Sin[\[Beta]/2]*((-30 + 7*E^l*(-225 + 4*ss^2))*
       h1[l] + 420*E^l*Derivative[1][h1][l]) + 
    (I/60)*E^(-l + (6*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^12*
     b\[Psi]l1**\[Psi]r1*((-6*(5 + E^l*(-225 + 4*ss^2)) + 
        (-30 + 7*E^l*(-225 + 4*ss^2))*Cos[\[Beta]])*h1[l] + 
      60*E^l*(-6 + 7*Cos[\[Beta]])*Derivative[1][h1][l]), 15/2, 13/2}, 
  {E^(-1/2*l + (7*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^14*
     (8*h1[l] - Derivative[1][h1][l]) - 
    E^(-1/2*l + (7*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^14*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     (8*h1[l] - Derivative[1][h1][l]) + 
    (I/16)*E^(-l + ((15*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^15*
     b\[Psi]l2**\[Psi]r2*((-16 + 15*E^l*(-64 + ss^2))*h1[l] + 
      240*E^l*Derivative[1][h1][l]) - 
    (I/16)*E^(-l + (I/2)*(13*\[Alpha] + 15*\[Gamma]))*Cos[\[Beta]/2]^14*
     b\[Psi]l1**\[Psi]r2*Sin[\[Beta]/2]*((-16 + 15*E^l*(-64 + ss^2))*h1[l] + 
      240*E^l*Derivative[1][h1][l]) + 
    (I/16)*E^(-l + (I/2)*(15*\[Alpha] + 13*\[Gamma]))*Cos[\[Beta]/2]^14*
     b\[Psi]l2**\[Psi]r1*Sin[\[Beta]/2]*((-16 + 15*E^l*(-64 + ss^2))*h1[l] + 
      240*E^l*Derivative[1][h1][l]) + 
    (I/32)*E^(-l + ((13*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^13*
     b\[Psi]l1**\[Psi]r1*((-16 - 13*E^l*(-64 + ss^2) + 
        (-16 + 15*E^l*(-64 + ss^2))*Cos[\[Beta]])*h1[l] + 
      16*E^l*(-13 + 15*Cos[\[Beta]])*Derivative[1][h1][l]), 8, 7}, 
  {(E^(-1/2*l + ((15*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^15*
      (17*h1[l] - 2*Derivative[1][h1][l]))/2 - 
    (E^(-1/2*l + ((15*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^15*
      b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
      (17*h1[l] - 2*Derivative[1][h1][l]))/2 + 
    (I/17)*E^(-l + (8*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^16*
     b\[Psi]l2**\[Psi]r2*((-17 + 4*E^l*(-289 + 4*ss^2))*h1[l] + 
      272*E^l*Derivative[1][h1][l]) - 
    (I/17)*E^(-l + (7*I)*\[Alpha] + (8*I)*\[Gamma])*Cos[\[Beta]/2]^15*
     b\[Psi]l1**\[Psi]r2*Sin[\[Beta]/2]*((-17 + 4*E^l*(-289 + 4*ss^2))*
       h1[l] + 272*E^l*Derivative[1][h1][l]) + 
    (I/17)*E^(-l + (8*I)*\[Alpha] + (7*I)*\[Gamma])*Cos[\[Beta]/2]^15*
     b\[Psi]l2**\[Psi]r1*Sin[\[Beta]/2]*((-17 + 4*E^l*(-289 + 4*ss^2))*
       h1[l] + 272*E^l*Derivative[1][h1][l]) + 
    (I/68)*E^(-l + (7*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^14*
     b\[Psi]l1**\[Psi]r1*((-34 - 7*E^l*(-289 + 4*ss^2) + 
        (-34 + 8*E^l*(-289 + 4*ss^2))*Cos[\[Beta]])*h1[l] + 
      68*E^l*(-7 + 8*Cos[\[Beta]])*Derivative[1][h1][l]), 17/2, 15/2}, 
  {E^(-1/2*l + (8*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^16*
     (9*h1[l] - Derivative[1][h1][l]) - 
    E^(-1/2*l + (8*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^16*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     (9*h1[l] - Derivative[1][h1][l]) + 
    (I/18)*E^(-l + ((17*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^17*
     b\[Psi]l2**\[Psi]r2*((-18 + 17*E^l*(-81 + ss^2))*h1[l] + 
      306*E^l*Derivative[1][h1][l]) - 
    (I/18)*E^(-l + (I/2)*(15*\[Alpha] + 17*\[Gamma]))*Cos[\[Beta]/2]^16*
     b\[Psi]l1**\[Psi]r2*Sin[\[Beta]/2]*((-18 + 17*E^l*(-81 + ss^2))*h1[l] + 
      306*E^l*Derivative[1][h1][l]) + 
    (I/18)*E^(-l + (I/2)*(17*\[Alpha] + 15*\[Gamma]))*Cos[\[Beta]/2]^16*
     b\[Psi]l2**\[Psi]r1*Sin[\[Beta]/2]*((-18 + 17*E^l*(-81 + ss^2))*h1[l] + 
      306*E^l*Derivative[1][h1][l]) + 
    (I/36)*E^(-l + ((15*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^15*
     b\[Psi]l1**\[Psi]r1*((-3*(6 + 5*E^l*(-81 + ss^2)) + 
        (-18 + 17*E^l*(-81 + ss^2))*Cos[\[Beta]])*h1[l] + 
      18*E^l*(-15 + 17*Cos[\[Beta]])*Derivative[1][h1][l]), 9, 8}, 
  {(E^(-1/2*l + ((17*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^17*
      (19*h1[l] - 2*Derivative[1][h1][l]))/2 - 
    (E^(-1/2*l + ((17*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^17*
      b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
      (19*h1[l] - 2*Derivative[1][h1][l]))/2 + 
    (I/38)*E^(-l + (9*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^18*
     b\[Psi]l2**\[Psi]r2*((-38 + 9*E^l*(-361 + 4*ss^2))*h1[l] + 
      684*E^l*Derivative[1][h1][l]) - 
    (I/38)*E^(-l + (8*I)*\[Alpha] + (9*I)*\[Gamma])*Cos[\[Beta]/2]^17*
     b\[Psi]l1**\[Psi]r2*Sin[\[Beta]/2]*((-38 + 9*E^l*(-361 + 4*ss^2))*
       h1[l] + 684*E^l*Derivative[1][h1][l]) + 
    (I/38)*E^(-l + (9*I)*\[Alpha] + (8*I)*\[Gamma])*Cos[\[Beta]/2]^17*
     b\[Psi]l2**\[Psi]r1*Sin[\[Beta]/2]*((-38 + 9*E^l*(-361 + 4*ss^2))*
       h1[l] + 684*E^l*Derivative[1][h1][l]) + 
    (I/76)*E^(-l + (8*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^16*
     b\[Psi]l1**\[Psi]r1*((-38 - 8*E^l*(-361 + 4*ss^2) + 
        (-38 + 9*E^l*(-361 + 4*ss^2))*Cos[\[Beta]])*h1[l] + 
      76*E^l*(-8 + 9*Cos[\[Beta]])*Derivative[1][h1][l]), 19/2, 17/2}, 
  {E^(-1/2*l + (9*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^18*
     (10*h1[l] - Derivative[1][h1][l]) - 
    E^(-1/2*l + (9*I)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^18*
     b\[Psi]l1**b\[Psi]l2**\[Psi]r2**\[Psi]r1*
     (10*h1[l] - Derivative[1][h1][l]) + 
    (I/20)*E^(-l + ((19*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^19*
     b\[Psi]l2**\[Psi]r2*((-20 + 19*E^l*(-100 + ss^2))*h1[l] + 
      380*E^l*Derivative[1][h1][l]) - 
    (I/20)*E^(-l + (I/2)*(17*\[Alpha] + 19*\[Gamma]))*Cos[\[Beta]/2]^18*
     b\[Psi]l1**\[Psi]r2*Sin[\[Beta]/2]*((-20 + 19*E^l*(-100 + ss^2))*h1[l] + 
      380*E^l*Derivative[1][h1][l]) + 
    (I/20)*E^(-l + (I/2)*(19*\[Alpha] + 17*\[Gamma]))*Cos[\[Beta]/2]^18*
     b\[Psi]l2**\[Psi]r1*Sin[\[Beta]/2]*((-20 + 19*E^l*(-100 + ss^2))*h1[l] + 
      380*E^l*Derivative[1][h1][l]) + 
    (I/40)*E^(-l + ((17*I)/2)*(\[Alpha] + \[Gamma]))*Cos[\[Beta]/2]^17*
     b\[Psi]l1**\[Psi]r1*((-20 - 17*E^l*(-100 + ss^2) + 
        (-20 + 19*E^l*(-100 + ss^2))*Cos[\[Beta]])*h1[l] + 
      20*E^l*(-17 + 19*Cos[\[Beta]])*Derivative[1][h1][l]), 10, 9}}}

